Probabilistic Conformance for Cyber-Physical Systems

In system analysis, conformance indicates that two systems simultaneously satisfy the same set of specifications of interest; thus, the results from analyzing one system automatically transfer to the other, or one system can safely replace the other in practice. In this work, we study the probabilistic conformance of cyber-physical systems (CPS). We propose a notion of (approximate) probabilistic conformance for sets of complex specifications expressed by the Signal Temporal Logic (STL). Based on a novel statistical test, we develop the first statistical verification methods for the probabilistic conformance of a wide class of CPS. Using this method, we verify the conformance of the startup time of the widely-used full and simplified model of Toyota powertrain systems, the settling time of model-predictive-control-based and neural-network-based automotive lane-keeping controllers, as well as the maximal voltage deviation of full and simplified power grid systems.

==> abs.tex <==


\title{Verification of Probabilistic Conformance for Cyber-physical 
Systems%
% \thanks{Supported by organization x.}%
}
% \titlerunning{Verification of Probabilistic Conformance}
% If the paper title is too long for the running head, you can set
% an abbreviated paper title here


% \author{Yu Wang\inst{1}\orcidID{0000-0002-0431-1039} \and
% Mojtaba Zarei\inst{1}\orcidID{1111-2222-3333-4444} \and
% Borzoo Bonakdarpoor\inst{2}\orcidID{2222--3333-4444-5555} \and
% Miroslav pajic\inst{1}\orcidID{2222--3333-4444-5555}}
% %
% \authorrunning{Wang et al.}
%\author{Anonymized Authors}


% \institute{Duke University, Durham NC 27707, USA
% \email{\{yu.wang094,mojtaba.zarei,miroslav.pajic\}@duke.edu}\\
% \and
% Iowa State University, Ames, IA 50011, USA
% \email{borzoo@iastate.edu}}
%\institute{Anonymized Affiliations}




\maketitle              % typeset the header of the  contribution
%
\begin{abstract}

{\em Conformance} is a key concept for the analysis of cyber-physical systems 
(CPS).
%
Roughly, it means that two models, derived either from the same system under 
two different conditions or two different systems under the same condition,
simultaneously satisfy the same specification of interest. The practical 
implication of conformance is that the result for analyzing one model 
with respect to the specification automatically transfers to the other.
%
In this paper, we propose a new concept for {\em probabilistic} conformance in 
CPS, extending the study of conformance testing to the probabilistic 
domain.
%
Specifically, probabilistic conformance of two models
is defined by the equal satisfaction probabilities
with respect to a given parameterized specification in the signal temporal 
logic.
%
In addition, we propose a statistical verification algorithm
for the probabilistic conformance of {\em grey-box} CPS. 
%
Based on the classic Kolmogorov-Smirnov test, we introduce a novel statistical test to check if two probability distributions are approximately equal for any desired confidence level ($< 1$).
%
We apply our technique to verify probabilistic conformance of 
(1) the startup time of the 
full and simplified models of the Toyota Powertrain system,
%
(2) the settling time of a model predictive control based 
lane-keeping controller and several neural network based lane-keeping controllers of different sizes for an autonomous car, and
%
(3) the maximal deviation of DC voltage between
the full and the simplified models of a
power grid system.


% \keywords{Statistical model checking \and Nonparametric statistical test \and 
% Probabilistic models.}

\end{abstract}

==> applications.tex <==
\begin[$(T, J, (\tau, \varepsilon))$-closeness]{definition}
For a time horizon $(T,J) \in \in R_+ \times \nat$, and parameters $\tau, \varepsilon > 0$. 
%
Two hybrid trajectories $\mu = (y; t; j)$ are
(T; J; (τ; "))-close, which we write µ ≈(τ;") µ0, if
(a) for all i 2 [N] such that t(i) ≤ T; j(i) ≤ J, there exists
k 2 [N0] such that j(i) = j0(k); jt(i) − t0(k)j < τ, and
ky(i) − y0(k)k < "
(b) for all i 2 [N0] such that t0(i) ≤ T; j0(i) ≤ J, there
exists k 2 [N] such that j0(i) = j(k); jt0(i) − t(k)j < τ, and
ky0(i) − y(k)k < "
The infimum of all " such that µ and µ0 are (T; J; (τ; "))-close
is called the achievable closeness degree given τ.
\end{definition}
